Comparison of Bayesian inference methods using the Loreli II database of hydro-radiative simulations of the 21-cm signal

While the observation of the 21 cm signal from the Cosmic Dawn and Epoch of Reionization is an instrumental challenge, the interpretation of a prospective detection is still open to questions regarding the modelling of the signal and the Bayesian inference techniques that bridge the gap between theory and observations. To address some of these questions, we present Loreli II, a database of nearly 10 000 simulations of the 21 cm signal run with the Licorice 3D radiative transfer code. With Loreli II, we explore a 5-dimensional astrophysical parameter space where star formation, X-ray emissions, and UV emissions are varied. We then use this database to train neural networks and perform Bayesian inference on 21 cm power spectra affected by thermal noise at the level of 100 hours of observation with the Square Kilometer Array. We study and compare three inference techniques : an emulator of the power spectrum, a Neural Density Estimator that fits the implicit likelihood of the model, and a Bayesian Neural Network that directly fits the posterior distribution. We measure the performances of each method by comparing them on a statistically representative set of inferences, notably using the principles of Simulation-Based Calibration. We report errors on the 1-D marginalized posteriors (biases and over/under confidence) below $15 \%$ of the standard deviation for the emulator and below $25 \%$ for the other methods. We conclude that at our noise level and our sampling density of the parameter space, an explicit Gaussian likelihood is sufficient. This may not be the case at lower noise level or if a denser sampling is used to reach higher accuracy. We then apply the emulator method to recent HERA upper limits and report weak constraints on the X-ray emissivity parameter of our model.

==> ch2/ch2_main.tex <==
\chapter{ Numerical modelling of the 21-cm signal}\label{chp2_chap}
\objectif{ In this chapter, we provide an overview of the numerical methods we use to simulate Reionization. In particular, we extensively discuss the \textsc{Licorice} simulation code, which is the main tool used during this work. Naturally, not all that is presented here is original work. My additions to \textsc{Licorice} are mainly the subgrid models for star formation and neutral temperature evolution, two crucial elements for realistic low-cost simulations which required significant modifications of the simulation code. The code was then used to produce the \textsc{\textsc{Loreli}} I and II databases, suites of simulations that we exploit for the inference task, as discussed in the next chapter. The code modifications and \textsc{\textsc{Loreli}} I are discussed in a published paper, \cite{Meriot2024}, while \textsc{\textsc{Loreli}} II and its exploitation will be the content of a soon-to-be-submitted follow-up paper. Additionally, part of \cite{Semelin2023} relies on low-cost \textsc{Licorice} simulation that I ran using the modified version of the code.  }



\section{A brief overview of numerical methods used to simulate the EoR}



As discussed in the previous chapter, the 21-cm signal is driven by various astrophysical processes, occurring over different time scales and coupling different spatial scales. As such, it is a complex numerical problem, and different strategies have been devised by the 21-cm community to try to accurately model the signal within reasonable computation constraints. Let us mention a few examples, categorized depending on their computational requirements.


\subsection{Semi-numerical methods}

Semi-numerical simulations are the fastest models of Reionization and the 21-cm. The most famous and widely adopted representant of these codes is 21cmFAST \citep{Mesinger2007,Murray2020},  typically able to generate a $512^3$ cube of 21-cm in a matter of hours.  To reach this low computation cost, some approximations and compromises must be made. 

In order to simulate Reionization, 21cmFAST first extrapolate a dark matter density field from initial conditions using the Zel'dovich approximation \citep{Zeldovich1970}. Hydrodynamics of the gas is neglected and baryons are assumed to perfectly trace dark matter. 

The most important simplification that semi-numerical models must make for the sake of speed is to not solve radiative transfer and instead produce ionization and gas temperature fields using photon budget estimates not unlike what is described at the end of section \ref{sec:UV}. 21cmFAST does not resolve ionizing sources, it computes for each cell of the grid the collapse fraction $f_{coll}$ using a Press-Schechter halo mass function (renormalized to match the more accurate Sheth-Tormen mass function, see section \ref{sec:cmf}), ascribes a stellar fraction to the unresolved dark matter halos that $f_{coll}$ represents, and uses the result to find the number of ionizing photons produced by the unresolved sources. These photons are not propagated. For instance, in \cite{Mesinger2007}, the code estimates the region that should be ionized by the sources. To do so, $f_{coll}$ is computed successively over decreasing scales starting from a horizon or mean free path parameter, and the code identifies the largest ionized region following \eqref{eq:semi_ion}\footnote{albeit with a slightly different parametrization for the ionizing efficiency.}   In a more recent version of the code \citep{Park2018, Sobacchi2014}, the smoothing scale starts at the box size, and if it reaches the cell length, a ionization fraction is computed. Similarly, the contribution of X-ray photons is estimated by assuming a spherically symmetrical heating by unresolved sources, proportional to $f_{coll}$. Lyman-$\alpha$ radiative transfer is handled with a similar approximation. As shown in \cite{Mesinger2007}, these approximations do have an impact on the morphology of the 21-cm field, and for example lead to ionized bubbles visibly more spherical compared to the results of full simulations.  

21cmFAST is not the only code in this category. For instance, the model used in \cite{Cohen2020} and references therein uses a different parametrization but relies on similar assumptions and simplifications.

The efficiency of these models is an asset : they are fast enough to be directly used in an MCMC inference pipeline \citep{Greig2015}, and can be used to explore high-dimensional parameter spaces and exotic effects (see e.g. \cite{Reis2021, Fialkov2019, Fialkov2018}) not implemented in more expensive codes that, due to computation costs, must limit their efforts to standard models.


\subsection{1D radiative transfer numerical simulations}

While semi-numerical codes estimate the contributions of sources they do not resolve, another approach is to rely on pre-ran N-body dark matter simulations to resolve the dark matter halos that are expected to contribute to reionisation, populate them with sources and compute their effect on the IGM in a post-processing step. This is done by using 1D ionization, Lyman-$\alpha$ and temperature profiles, which must only be computed once for a given cosmology and source model. 
Using the source catalogue of the N-body simulation (or, more accurately, their star formation histories), the right 1D profiles are selected and painted on the 3D grid. This approach is at the heart of e.g. Grizzly \citep{Ghara2018} and Beorn \citep{Schaeffer2023}, and there again, the strategy is to avoid the cost of full 3D radiative transfer while hopefully benefitting from a more accurate source distribution and modelling than in faster semi-numerical code. These codes typically yield a 21-cm signal in a few CPU-hours, at a $256^3$ resolution (e.g. \cite{Ghara2018}).  


\subsection{3D radiative transfer simulations}

Finally, part of the EoR community focused on producing simulations that include computationally expensive but  accurate 3D radiative transfer. Amongst these codes, we can (non-exhaustively) list Coda \citep{Lewis2021}, C$^2$-ray \citep{Mellema2006}, Thesan \citep{Smith2022, Garaldi2022, Kannan2022}, EMMA \citep{Aubert2015} and the one used in this work, \textsc{Licorice} \citep{Meriot2024}. In principle, they simulate the non-linear evolution of the density field, identify star forming regions, and proceed to propagate photons and solve the 3D radiative transfer equations to simulate the evolution of the ionization and temperature of the IGM. In addition, the radiative transfer is ideally coupled to the gas, meaning that the hydrodynamics of the gas depend on its physical state, and therefore of the radiation field produced by the sources, the formation of which depend on the hydrodynamics. Different radiative transfer methods exist, mainly the moments method \citep{Aubert2008} (in short, a hydrodynamical formulation of the behavior of the radiation field, assumed to be a "pseudo-fluid")  and ray-tracing \citep{Abel1999} (a large number of photon packets are emitted by the sources, are individually tracked by the code, and interact with the IGM as they travel). The former is faster and scales well with the number of sources, but produces some unphysical results (see e.g \cite{Aubert2008, Gnedin2001, Hayes2003}), while the latter can be more accurate, but also more expensive and, in the Monte Carlo ray-tracing scheme, introduces a form of noise in the results, as the radiation field is sampled by a finite number of rays.



It would be dishonest to pretend that these codes do not contain any approximation. For instance, the simulated volume required to capture the large scale fluctuations of the 21-cm is of the order of a Gpc, while the individual stars and AGNs formed in sub-parsec scales that are naturally not resolved, and neither are some feedback effects that regulate star formation. Hence, while they attempt to model Reionization from first principles as much as possible, the simulations must also rely on sub-grid star formation recipe, source models, and ad-hoc parameters such as the escape fraction of ionizing radiation. Some approaches to hydrodynamics also suffer from the wide range of scales at play in the 21-cm problem. For example, smooth-particle hydrodynamics (SPH, see next chapter) includes an artificial viscosity to properly account for shocks in the gas. Numerical difficulties also arise in the coupling of the gas dynamics to the radiative transfer, as both phenomena involve different typical spatial and temporal scales. 



Note that although 3D radiative transfer simulations include fewer approximations than semi-numerical codes, the sheer amount of computation time required prevents the community from using them in many circumstances. All the approaches presented here are complementary : expensive simulations may be used as reference to calibrate faster ones, which can then be used to explore high dimensional parameter spaces. However, while a few attempts have been made to compare different codes  (see e.g. \cite{Hutter2018, Ghara2018, Zahn2010, Iliev2006a}), the different parametrizations used by the different codes prevent accurate one-to-one comparisons. Thus, the community has not identified a single clearly superior method, and for the foreseeable future observations will be interpreted using a diversity of approaches, hopefully leading to some form of consensus.


This work relies exclusively on \textsc{Licorice}, a 3D radiative transfer code which we extensively describe in this chapter. 



%\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ The \textsc{Licorice} simulation code }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textsc{Licorice} is a High Performance Computing hydro-radiative code that aims to simulate the dark ages, the Cosmic Dawn, and the EoR, in order to provide accurate predictions of the 21-cm signal. It has been developed at LERMA for more than a decade, and details and evolution of the codes can be found in \cite{Meriot2024, Semelin2017, Baek2009, Semelin2007} (and references therein). It consists in simulating the dynamics of dark matter and baryonic matter (gas) particles. The code tracks the physical properties of the latter, and they evolve in a box with periodic boundary conditions. In order to run on national supercomputers, the code is parallelized with both OpenMP and MPI. 


To properly simulate the EoR, the code must couple different physical processes : it must solve gravity, update the positions and velocities of particles, update the relevant physical quantities, simulate structure formation (i.e. form stars). Once stars exist in the simulation, it must also emit new photons in the relevant bands, propagate in-flight photons, solve radiative transfer and process the interaction of photons with the gas they encounter. In practice, \textsc{Licorice} operates by interconnecting different modules, which we describe in the following.

\subsection{Efficiently solving gravity : the Tree code}

\begin{figure}[H]\centering
\includegraphics[scale = 0.3]{ch2/fig/BarnesHut_example.jpg}
\caption{Illustration of the Tree algorithm for computing gravity. The force to estimate is the one applied to the red particle, and the groups left unopened and for which  the multipole expansion of the force is computed are in orange. From \url{ https://anaroxanapop.github.io/behalf/}}
\label{fig:tree}
\end{figure}


The range of gravity is infinite, therefore a simulation code dealing with $N$ particles has to deal with $\frac{N \times (N-1)}{2}$ gravitational interactions. A naive implementation would cause the code to scale with $O(N^2)$. This inefficient scaling has led researchers to design approximate but faster prescriptions for gravity in cosmological settings. The one used in \textsc{Licorice} is the Tree approach \cite{Appel1985, Barnes1986}, which first organizes particles in groups by first subdividing the simulation box into 8 smaller cubic boxes called cells. Then, each cell is in turn subdivided in 8 smaller cells, recursively, until each cell contains either 0 or 1 particle. To compute the total gravitational force applied on a particle, the exact interaction is only calculated for nearby particles. The interactions with distant particles (those in groups seen with an angle smaller than some numerical parameter $\theta$) are not directly calculated : they are replaced by the multipole expansion of the gravitational force exerted by the group to which they belong.  In practice, \textsc{Licorice} performs the expansion up to the quadrupole only. Averaging the contribution of distant particles in such a way allows for a $O(NlogN)$ scaling. At high redshift, the relative error in the computation of the forces by the Tree code becomes significant, as the density field is homogeneous and the total force applied on a particle is small. To mitigate this, the effective $\theta$ parameter is smaller at $z < 30$, allowing a more accurate (but more expensive) force computation. Figure \ref{fig:tree} shows an illustration of the Tree algorithm. 
Because \textsc{Licorice} is parallelized with MPI, the largest cells of the Tree are the MPI domains themselves.
In practice, each domain constructs its own tree, to which it adds the trees of the adjacent domains. Non-adjacent domains are never opened and are always represented by the multipole expansion of the gravitational force, and domains are themselves assembled in their own tree. 


\subsection{Gas dynamics : the Smoothed Particle Hydrodynamics algorithm}

The computation of gravitational force is sufficient to know the dynamics of collisionless matter, i.e. the dark matter particles. However, gas is not collisionless and needs a numerical treatment of hydrodynamics. We use a prescription of the Smoothed Particle Hydrodynamics Lagrangian approach, which we briefly describe here.
As the name indicates, the physical properties of a particle indexed by $i$ are smoothed over some length  $h_i$. This smoothing length is defined as the radius that encompasses the $N_{near}$ nearest neighbours of the particle $i$, and finding these neighbours can be computationally expensive. Fortunately, the Tree constructed in the previous step is a powerful tool : all the particles contained in cells that lie completely within some predetermined search volume are added to the neighbours list, and cells that only overlap with the search volume are opened in order to apply the same process to their descendants. In order to keep the number of neighbours $N^{(t)}$ approximately constant and close to $N_{near}$ between a time step $t$ and the next, the comoving search radius $h_i$ must be carefully designed. The following equation is used to compute $h_i^{(t+1)}$ given $h_i^{(t)}$ and  $N^{(t)}$ :

%, and the velocity divergence $ (\nabla \cdot v)_i$
% \begin{equation}
%         h_i^{(t+1)} =  \frac{1}{2}  h_i^{(t)} \left( 1 +  \left( \frac{N_{near}}{N^{(t)}} \right)^{1/3}   \right) +  \frac{1}{3}  h_i^{(t)} (\nabla \cdot v)_i \Delta t
% \end{equation}


\begin{equation}
        h_i^{(t+1)} =  \frac{1}{3}  h_i^{(t)} \left( 1 +  3\left( \frac{N_{near}}{N^{(t)}} \right)^{1/3}   \right) 
\end{equation}

\noindent where the term in brackets tends to bring  $N^{(t+1)}$ back closer to $N_{near}$, should $N^{(t)}$ have diverged from it. For discussion surrounding the update of smoothing length, see e.g. \cite{Springel1998} (and references therein). Note that fluctuations in $N_{near}$ add variance to the quantities estimated by SPH without affecting their expected value. In practice, $N_{near}$ is set to $30$ and the number of neighbours observed in the simulations remains satisfyingly close to it.

For a given particle $i$, once $h_i$ has been calculated and its neighbours $(N_j)_{1\leq j \leq n}$ have been found, its comoving density $\rho_i$ can be computed as 

 \begin{equation}
     \rho_i = \sum_ {j=1}^n m_j W(r_{ij}, h_i)
 \end{equation}

 \noindent where $m_j$ is the mass of the neighbour particle $N_j$, $r_{ij}$ the comoving distance between the particle $i$ and its neighbour $N_j$, and $W$ the kernel used to smooth over the density field sampled by the particles. We use the spherically symmetric spline kernel function proposed by \cite{Monaghan1985}   : 

 \begin{equation}\label{eq:sphkern}
     W(r,h) =     \begin{cases}
      \frac{8}{\pi h^3} ( 1- 1.5 \left( \frac{2r}{h} \right)^2  + 0.75 \left( \frac{2r}{h} \right)^3   )  & \text{if $r < 0.5h$ }\\
       \frac{8}{ \pi h^3} ( 0.25 * (2 - \left( \frac{2r}{h} \right) )^3   & \text{if  $0.5h \leq r < h$ }\\
      0 & \text{otherwise}
    \end{cases}
 \end{equation}

 Gas particles are assumed to behave like an ideal gas, therefore their pressure $P_i$ is set depending on their density, their internal energy $u_i$, and the ideal gas heat capacity ratio $\gamma$ : $P_i = (\gamma - 1) \rho_i u_i/a^3$. This finally allows for the computation of the total force applied to a particle $i$ :

 % \begin{equation}
 %    % m_i a_i =  \sum_k G_{ki}  -\sum_ {j=1}^n (1-f_{*,j})m_j \left( \frac{2}{a^3}\sqrt{\frac{P_i}{\rho_i } \frac{P_j}{\rho_j }} + \Pi_{ij} \right)   \frac{\partial W}{\partial r} (r_{ij} ,h_i) \frac{1}{r_{ij} a^5}
 %        m_i a_i =  \sum_k G_{ki}  -\sum_ {j=1}^n (1-f_{*,j})m_j \left( \frac{2}{a^3}\sqrt{\frac{P_i}{\rho_i } \frac{P_j}{\rho_j }} + \Pi_{ij} \right)   \nabla_i W(r_{ij} ,h_i) \frac{1}{r_{ij} a^5}
 % \end{equation}

 \begin{equation}
    % m_i a_i =  \sum_k G_{ki}  -\sum_ {j=1}^n (1-f_{*,j})m_j \left( \frac{2}{a^3}\sqrt{\frac{P_i}{\rho_i } \frac{P_j}{\rho_j }} + \Pi_{ij} \right)   \frac{\partial W}{\partial r} (r_{ij} ,h_i) \frac{1}{r_{ij} a^5}
        m_i a_i =  \sum_k G_{ki}  -\sum_ {j=1}^n (1-f_{*,j})m_j \left( \frac{2}{a^3}\sqrt{\frac{P_i}{\rho_i } \frac{P_j}{\rho_j }} + \Pi_{ij} \right)  \frac{d}{dr} [W(r_{ij} ,h_i)] \frac{1}{ a^4} \frac{r_{ij}}{|r_{ij}|}
 \end{equation}


\noindent where $\sum_k G_{ki}$ represents the sum of the  gravitational interactions applied to $i$ calculated in the previous section, $a_i$ the acceleration of particle $i$ in physical coordinates,  $a$ the expansion factor of the universe, $f_{*, j}$ the stellar fraction\footnote{The fraction of the mass of the particles that is in stars and not non-collapsed gas; more details in section \ref{sec:cmf}.} of the particle $N_j$, and  $ \Pi_{ij}$ is an artificial viscosity term introduced by   \cite{Monaghan1992} that is necessary for SPH implementations to properly take shocks into account. We use the expression presented in \cite{Springel2005}, adapted to an expanding universe :

\begin{equation}
     \Pi_{ij} = \begin{cases}

       \frac{- \mu_{ij}c_{ij} + \mu_{ij}^2  }{ 0.5(\rho_i + \rho_j)a^3 }   & \text{if  $v_{ij} \cdot r_{ij} < 0$ }\\
      0 & \text{otherwise}
    \end{cases}
\end{equation}

\noindent where $c_{ij}$ is the arithmetic average of the sound speeds in particles $i$ and $N_j$, $v_{ij}$ their relative velocities, and 

 \begin{equation}
     \mu_{ij} = \left( \frac{h_i + h_j}{2} \right) \left( \frac{v_{ij} \cdot r_{ij}a^2 + a \Dot{a} r_{ij}^2  }{a r_{ij}^2} \right) .
 \end{equation}



Similarly, the equation governing the evolution of the internal energy of the particle is

 % \begin{equation}\label{eq:dudt}
 %      \frac{{\rm{d}}u_i}{\rm{dt}}   =  \frac{1}{2}\sum_ {j=1}^n (1-f_{*,j})m_j \left( \frac{2}{a^3}\sqrt{\frac{P_i}{\rho_i } \frac{P_j}{\rho_j }} + \Pi_{ij} \right) \frac{1}{|r_{ij}| a^5}  v_{ij} \cdot \nabla_i W(r_{ij} ,h_i) + \Lambda = K + \Lambda
 % \end{equation}


  \begin{equation}\label{eq:dudt}
      \frac{{\rm{d}}u_i}{\rm{dt}}   =  \frac{1}{2}\sum_ {j=1}^n (1-f_{*,j})m_j \left( \frac{2}{a^3}\sqrt{\frac{P_i}{\rho_i } \frac{P_j}{\rho_j }} + \Pi_{ij} \right)    \frac{d}{dr} [W(r_{ij} ,h_i)] \frac{ v_{ij} \cdot r_{ij}a^2 + a \Dot{a} r_{ij}^2  }{|r_{ij}| a^5}  + \Lambda = K + \Lambda
 \end{equation}

\noindent where $\Lambda$ represents heating and cooling caused by e.g. radiative transfer which will be detailed in a subsequent section, and $K$ represents the sum in the above equation, i.e. only the adiabatic evolution of the gas.\\


To update the positions $r_i$ and velocities $v_i$ of the particles, the code relies on a leap frog integrator, here again adapted to an expanding universe. First, the positions of the particles after half a time step are predicted : 
\begin{equation}
    r_i^{(t + 1/2)}=r_i^{(t)} + \frac{\Delta t_{dyn}}{2} v_i^{(t)}
\end{equation}
At this position, the acceleration of the particle $a_i^{(t + 1/2)}$ is computed following the procedure previously described. Finally, the positions and velocities of the particles after a full time step are computed \footnote{Beware : $a_i$ denotes the acceleration of the particle $i$ while $a$ denotes the scale factor of the universe} :
\begin{equation}
    v_i^{(t+1)} = v_i^{(t)} +   \left( \frac{1}{a} a_i^{(t + 1/2)} - 2 \frac{\Dot{a}}{a}v_i^{(t)}  \right) \Delta t_{dyn}
\end{equation}
\begin{equation}
    r_i^{(t+1)} = r_i^{(t)} +   \frac{1}{2} \left( v_i^{(t)} + v_i^{(t + 1/2)} \right) \Delta t_{dyn}
\end{equation}


\subsection{Star formation and the Conditional Mass Function formalism}\label{sec:cmf}

\subsubsection{ The Conditional Mass Function }



The next challenge that the simulation code must face is the one of structure formation. Indeed, the birth and life of stars, globular clusters, proto-galaxies and small galaxies, consist of phenomena that occur on scales that are tiny compared to the size of the cosmological box and cannot be entirely resolved. One must rely on aptly designed numerical recipes to represent them. As discussed in Chapter \ref{ch1}, star forming regions are expected to be the regions where gas undergoes gravitational collapse.  While it is tempting to directly apply Jeans instability criterion to particles in the simulation, softened gravity can lead to poor estimate of its validity \cite{Katz1992}. In addition, the gas cooling time must be shorter than the dynamical time associated with the collapse. In cosmological simulations, the issue can be simplified by assuming that these conditions are satisfied if the gas overdensity is higher than $\delta_{crit} \approx 200$ (e.g. \cite{Navarro1993, Doussot2022}), which is approximately the threshold above which a spherical density perturbation will collapse and often used to define a collapsed object. \\


Applying this criterion at the scale of the particle is sufficient only if the simulation has the resolution to resolve all the dark matter halos that are thought to contribute to Reionization, i.e. halo masses down to a few $10^8 \Msun$ {(see Chapter \ref{ch1})}. As it takes at least $\sim 20$ particles to properly identify a halo, resolving halos this small in a cosmological volume of $\sim (300 \Mpc)^3$ requires at least $4096^3$ particles. As \textsc{Licorice} simulations with $2048^3$ particles typically require a few million CPU-hours to run, using $4096^3$ particles is computationally expensive within current resources constraints. In order to save computation time and still obtain realistic star formation rates irrespective of resolution, we decided to implement a subgrid model for star formation that aims to statistically estimate the amount and mass of unresolved dark matter halos. This model relies on the Conditional Mass Function (CMF) formalism. It is an extension of the Halo Mass Function (HMF), a theoretical prediction for the abundance of dark matter halos on average in the Universe. The first, and arguably most widely used, HMF is the one derived by Press and Schechter \citep{Press1974},  which was shown to be qualitatively correct when compared to mass functions measured in N-body simulations  (but not perfect, see e.g. \cite{Reed2007}). While this was not the original approach, their result can be obtained following the excursion set formalism, crucial in the derivation of the CMF from the HMF, which we briefly summarize here. 


 First, as previously explained, we consider that an object is collapsed when its (non-linear) density exceeds some threshold $\delta_{crit}$. However, the  Press-Schechter approach relies on the linear theory of structure formation. Given a non-linear overdensity $\delta_{NL}$, one can infer a corresponding extrapolated linear overdensity $\delta_L$ through \ :

\begin{equation}
    \delta_L = \frac{\delta_c}{1.68647} \left(  1.68647 - \frac{1.35}{(1 + \delta_{NL})^{2/3}}  - \frac{1.12431}{(1 + \delta_{NL})^{1/2}}  + \frac{0.78785}{(1 + \delta_{NL})^{0.58661}} \right)
\end{equation}

\noindent where $\delta_c \approx 1.68647$ is the linear threshold for collapse \citep{Sheth}.

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.5]{ch2/fig/random_walk.png}
    \caption{Illustration of the random walk approach to structure formation. By successively smoothing the density field around the same position over decreasing radii ($R_1 > R_2 > R_3$), the resulting smoothed linear overdensity follows a random walk. In this illustration, the walk crosses the $\delta_c \approx 1.68$ threshold at $R_3$, and we therefore consider that a halo of radius $R_3$ has been identified at this location. }
    \label{fig:random_walk}
\end{figure}




Now, let us consider that the density field is Gaussian, driven by a matter power spectrum $P_m$. The variance of the density field at a given scale $R$ is given by 

\begin{equation}
    \sigma^2(R,z) = \frac{1}{(2\pi)^3} \int P_m(k,z) W^2(k) d^3k
\end{equation}

\noindent where $W$ is a {window} function such that $W(k) \longrightarrow 0$ if $k \gg 2\pi/R$ and  $\int W(k){\rm{d}}k = 1$. Note that a given scale $R$ defines a mass $M$ through $M = \frac{4}{3}\pi \rho_0 R^3$.  Now let us consider a series of concentric spheres of decreasing radii centred around some position $x$. As the density field is Gaussian, the density fluctuation modes $\delta(k)$ of different $k$ are uncorrelated, therefore the series of overdensities associated with the spheres follows a random walk. Indeed, the evolution of the smoothed density between smoothing radii $R_1$ and $R_2$ depends on the realization of the random density field in the shell between $R_1$ and $R_2$, that is, in Fourier space, on the amplitudes and phases of the density modes on scales between $2\pi/R_2$ and $2\pi/R_1$. The probability of finding a halo with a mass between $M$ and $M+dM$ at $x$ is then given by the fraction of these linear densities random walks that cross the overdensity threshold $\delta_c$ for the first time between $R$ and $R + dR$ {(see illustration on Figure \ref{fig:random_walk})}, or, equivalently, between $\sigma$ and $\sigma - d\sigma$. Following  \cite{Lacey1993} and \cite{Chandrasekhar1943}, this random walk approach of the Press-Schechter (PS) mass function predicts a number density $n_{PS}(M)$ of halos with mass between $M$ and $M+dM$ :

\begin{equation}\label{eq:hmf_ps}
    n_{PS}(M) = \sqrt{\frac{2}{\pi}} \left| \frac{d\sigma}{dM} \right| \frac{\rho_0}{M} \frac{\delta_c}{\sigma(M,z)^2} {\rm{exp}} \left(- \frac{\delta_c^2}{2\sigma(M,z)^2}\right)
\end{equation}



Note that the evolution with redshift of the mass function is fully determined by the redshift dependence of $\sigma$, that is in turn given by the growth of the power spectrum $P_m$ with time :  

\begin{equation}
    P_m(k,z) = D(z)P_m(k,z = 0)
\end{equation}

\noindent where $D$ is the linear growth factor, normalized to unity at $z = 0$. Following e.g \cite{Hamilton2001} (and references therein), it solely depends on the chosen cosmology :

\begin{equation}
    D(z) \propto \frac{5}{2}\frac{ \Omega_m(z)}{\Omega_{m}^{0.57}(z) + \Omega_\Lambda(z) + \left(1 + \frac{\Omega_m(z)}{2}\right)\left(1+ \frac{\Omega_\Lambda(z)}{70}\right)  }
\end{equation}


\noindent with 

\begin{equation}
    \Omega_m(z) = \frac{\Omega_{m,0}(1+z)^{3}}{\Omega_{m,0} (1+z)^{3} + \Omega_{\Lambda,0} }
\end{equation}

\begin{equation}
    \Omega_\Lambda(z) = \frac{\Omega_{\Lambda,0}}{\Omega_{m,0} (1+z)^{3} + \Omega_{\Lambda,0} }
\end{equation}




\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.45]{ch2/fig/hmf.pdf}
    \caption{Evolution with redshift of the halo mass function of HIRRAH-21, calculated using a FoF algorithm. We also show the history of theoretical PS and ST HMFs for the same cosmology. Taken from  \cite{Meriot2024}.}
    \label{fig:hmf}
\end{figure}




Eq. \eqref{eq:hmf_ps} gives an estimate of the average halo population in the Universe. However, we are interested in the halo population found in a given region, characterized by a size $R_0$ and an overdensity $\delta_0$. As previously mentioned, specifying the size $R_0$ is equivalent to specifying $\sigma_0 = \sigma(R_0)$. With this approach, the CMF can be obtained from the HMF by simply rescaling the variables as

    \begin{equation}
\begin{split}
\delta_c & \rightarrow \delta_c - \delta_0   \\
 \sigma(M,z)^2 & \rightarrow  \sigma(M,z)^2 -  \sigma_0(z)^2
\end{split}
\end{equation}

\noindent {which represents the condition that the random walk starts from the position that describes the region and not the average Universe on infinitely large scales.} It yields the \textit{Extended Press-Schechter} CMF :

\begin{equation}\label{eq:cmf_eps}
    n_{EPS}(M) = \sqrt{\frac{2}{\pi}} \left| \frac{d\sigma}{dM} \right| \frac{\rho_0}{M} \frac{\sigma(\delta_c - \delta_0)}{ (\sigma^2 -  \sigma_0^2)^{3/2}} {\rm{exp}} \left(- \frac{\delta_c^2}{2(\sigma^2 -  \sigma_0^2)}\right)
\end{equation}


\noindent While straightforward to derive, the PS versions of the HMF and CMF are not the most accurate analytic prescription of the mass function. Its main caveat is that it assumes a spherical collapse. \cite{Sheth2001} (ST) improved it by including the physics of ellipsoidal collapse by changing the constant collapse threshold $\delta_c$ used during the random walk into a mass-dependent threshold given by : 

\begin{equation}
    B(\sigma^2, z)  = \sqrt{a}\delta_c[1 + \beta(a\frac{\delta_c^2}{\sigma^2})^{-\alpha}]
\end{equation}

\noindent where $a \approx 0.707$ is fitted to simulations and $\alpha  \approx 0.615, \beta  \approx 0.485$ are parameters derived from the dynamics of ellipsoidal collapse. This eventually yields a HMF : 







% \begin{equation}\label{eq:hmf_ST}
%     n_{ST}(M) = \sqrt{\frac{2}{\pi}} \left| \frac{d\sigma}{dM} \right| \frac{\rho_0}{M} \frac{|B(\sigma^2, z) | }{\sigma^2} {\rm{exp}} \left( -\frac{B(\sigma^2, z)^2}{2\sigma^2} \right)
% \end{equation}


\begin{equation}\label{eq:hmf_ST}
    n_{ST}(M) =  A \sqrt{\frac{2a}{\pi}} \left| \frac{d\sigma}{dM} \right| \frac{\rho_0}{M}  \left[1 + \left(\frac{\sigma^2}{a\delta_c^2}\right)^{0.3} \right]  \frac{\delta_c}{\sigma(M,z)^2} {\rm{exp}} \left(- \frac{a\delta_c^2}{2\sigma(M,z)^2}\right)
\end{equation}

\noindent {where $A \approx 0.3222$} and \cite{Rubino-Martin2008, Sheth} proposed a corresponding CMF, again using the substitution $B(\sigma^2, z)  \rightarrow B(\sigma^2, z) - \delta_0$ :

\begin{equation}\label{eq:st_cmf}
      n_{c, ST}(M) =  \sqrt{\frac{2}{\pi}} \left| \frac{d\sigma}{dM} \right| \frac{\rho_0}{M} \frac{|T(\sigma^2 | \sigma_0^2)|\sigma}{(\sigma^2- \sigma_0^2)^{3/2}} \rm{exp} \left( -\frac{(B(\sigma^2, z) - \delta_0)^2}{2(\sigma^2 - \sigma_0^2)} \right)
\end{equation}

\noindent  where 

\begin{equation}
    T(\sigma^2 | \sigma_0^2) = \sum^5_{n=0} \frac{(\sigma_0^2 - \sigma^2)^n}{n!} \frac{\partial^n[B(\sigma^2, z) - \delta_0]}{\partial(\sigma^2)^n}.
\end{equation}




In a given region of volume $V_{region} = \frac{4}{3}\pi R_0^3$ containing a mass $M_{region}$, one can integrate the CMF and obtain  an estimate of $M_{coll}$, the mass contained in collapsed structures more massive than some parameter $M_{min}$, as

\begin{equation}
      M_{coll} = V_{region} \int_{M_{min}}^{M_{region}}  n_c(M)M\rm{dM}
\end{equation}

\noindent as well as the collapsed fraction as

\begin{equation}\label{eq:fcoll2}
    f_{coll} =  \frac{M_{coll}}{M_{region}}.
\end{equation}

Conveniently, in the EPS formalism, the collapsed fraction has an analytical expression :

\begin{equation}\label{eq:fcoll}
    f_{coll} = \rm{erfc}\left[ \frac{\delta_c-\delta_0}{\sqrt{2(\sigma(M_{min})^2 - \sigma_0^2 })}\right]
\end{equation}


\noindent which is not the case in the ST approach.




\subsubsection{The star formation subgrid model}



For simplicity, we assume that the baryon-to-dark matter ratio in halos is the same as the cosmological ratio, {although it has been shown to  correlate with halo mass, see e.g. \cite{Henden2018, Davies2019}}. Therefore, $f_{coll}$ is also the fraction of the gas in the region that undergoes gravo-thermal collapse and plays a critical role in the star formation in the simulation. Indeed, in \textsc{Licorice}, the particles identified as collapsed form stars following a Schmidt law of exponent 1. In other words, $df_{*}$, the fraction of the gas particle converted into stellar mass during a time step $\Delta t_{dyn}$  is calculated as 

 \begin{equation}\label{eq:sf}
     df_{*} = (f_{coll} - f_{*})\dfrac{\Delta t_{dyn}}{\tau_{SF}}
 \end{equation}


\noindent where $f_*$ is the mass fraction of the baryon particle that belongs to stars, and $\tau$ the star formation timescale i.e. the typical duration over which collapsing gas is converted into stars; it encompasses all kinds of unresolved feedbacks. For a discussion on feedback at high redshift, see e.g. \cite{Klessen2023}. This is an active field of research, and the constant gas-to-dark matter ratio and mass-independent $\tau_{SF}$ are simple assumptions, but since the CMF formalism describes populations of halos we can expect them to hold on average. The term $(f_{coll} - f_{*})$ represents the gas reservoir in the particle that is yet to be converted into stars. Note that the two parameters of the model are $\tau_{SF}$ and $M_{min}$. \\





In practice, $f_{coll}$ is calculated for all gas particles in the simulation, either by applying the formula in Equation \eqref{eq:fcoll} in the EPS case or by computing and integrating the ST CMF in the ST case.  The local baryon-to-dark matter is always assumed to be at the cosmological value, meaning that $M_{region} = M_{gas} \times \Omega_m/\Omega_b$, the overdensity in the region (from which is derived the corresponding linear overdensity) is given by the SPH algorithm and the effective volume is calculated as  

\begin{equation}
   V_{region} = \gamma\frac{4}{3}\pi h^3
\end{equation}


\noindent where $h$ is the SPH smoothing radius previously described and  $\gamma$ a correction factor that arises from the fact that the region defined until now is defined under the assumption of a top-hat kernel, while the smoothing occurring in the SPH algorithm specifies a different kernel. In practice, the integral of the SPH kernel reaches $99\%$ of its maximum value at $ \sim 0.7 h$, therefore $\gamma \sim 0.4$  is a reasonable choice, but the parameter can be fine-tuned to reproduce the results of high-resolution simulations. \textit{In fine}, the implementation of this subgrid model increases the star formation in the simulation : it causes particles below the $\delta_{crit}$ threshold to still form significant amount of stars. Additionally, it smoothly transitions to the regime where the collapsed structures are resolved, since $f_{coll}$ approaches $1$ when the overdensity approaches $\delta_{crit}$.


\subsubsection{Performance of the subgrid model}


\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.42]{ch2/fig/cmf_delta_dependence.pdf}
    \caption{ Evolution of the simulated CMF with the overdensity $\delta$ and of the theoretical CMFs as predicted by the ST and EPS models. In order to match the high resolution simulation, the $\sigma$ in the EPS model has been scaled up by $5 \%$. From \cite{Meriot2024}.}
    \label{fig:cmf}
\end{figure}




To validate this approach, we first compare the theoretical predictions of the ST and PS HMF models to the dark matter halo mass function measured in HIRRAH-21, a $2048^3$ \textsc{Licorice} simulation presented in \cite{Doussot2022} in which halos down to masses of $ \sim 4 \times 10^9 \Msun$ are resolved (and from which the star formation subgrid model is absent). The HMF of HIRRAH-21 has been measured using a Friends-of-Friends algorithm on-the-fly in the simulations. The three HMFs are plotted on Figure \ref{fig:hmf} at different redshifts. The ST HMF demonstrates an excellent agreement with the one measured in HIRRAH-21, with residuals explainable by the Poisson noise induced by Cosmic Variance in the simulations. However, the PS mass function underestimates the halo abundance by an order of magnitude (or, equivalently, exhibits a delay in structure formation of $\Delta z \approx 2$ at the considered redshifts). Additionally, Figure \ref{fig:cmf} shows the EPS and ST CMF as well as the CMFs measured in HIRRAH-21 at $z\approx 9.5$ for different overdensities, in regions of radius $5 \Mpc$. Once again, the ST formalism agrees with the simulated results. However, to fit to the simulation, the EPS CMF was calculated
using a $10\%$ smaller radius  to define the particle volume. Even with this tuning, the EPS CMF diverges from the simulation at high masses and high overdensities, making it clear that an implementation relying on the ST CMF would produce better results.   Consequently, this is the implementation adopted in the following.

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.4]{ch2/fig/SFR_vs_z2048like_ST.pdf}
    \caption{History of the star formation rates of HIRRAH-21 and LORRAH-21. As a reference, observational data from \cite{Bouwens2016, Oesch2018, McLeod2016} is included. The SFRD of a $1024^3$ particles simulation is also plotted, and is consistent with that of a LORRAH-21 simulation using a $M_{min}$ parameter set at the value of the smallest resolved halos in the $1024^3$ simulation. \cite{Meriot2024}}
    \label{fig:sfr}
\end{figure}


However, with no subgrid model, star formation in \textsc{Licorice} does not necessarily occur in resolved halos {(identified e.g. by a halo finder)}, but in dense gas particles, {so matching halo mass functions does not immediately imply matching star formation}. As a final test, we compare the star formation rate densities (SFRD) in simulations of $256^3$ particles, with two simulations of  higher resolutions : HIRRAH-21, and one with $1024^3$ particles, (part of the 21SSD dataset, see \cite{Semelin2017}), that resolves dark matter halos down to $\sim 3 \times 10^{10} \Msun$. The initial density fields and cosmological parameters were kept the same in the high-resolution simulations and their low resolution counterparts, as were the astrophysical parameters ($\tau_{SF}$ in particular). The $M_{min}$ parameter in the subgrid model of low-resolutions simulations was set to the masses of the lightest resolved halos in the high-resolution ones, mentioned above. {We call LORRAH-21 the low-resolution counterpart to HIRRAH-21.

The results are shown on Figure \ref{fig:sfr}, and we observe an excellent agreement between the SFRD in high-resolution simulations and their low resolution counterparts. In particular, the results are not sensitive to resolution  and the SFRD in low-resolution simulations is as realistic in the $M_{min} = 3 \times 10^{10} \Msun $ case as it is in the  $M_{min} = 4 \times 10^{9} \Msun $ one, suggesting that it would perform as well with lower values of $M_{min}$, closer to what is expected in standard models of the EoR.
A final subtlety in the implementation, which may explain the discrepancy between the SFRD of high- and low-resolution simulation, remains. As will be detailed in the next section, all particles with a non-zero $f_*$ are considered sources. However, the subgrid model for star formation, as it is, always predicts a strictly positive $f_{coll}$. At high $z$ all gas particles will be affected with a strictly non-zero, although infinitesimal, $f_*$. This will cause the propagation of many photon packets early in the simulation, which is both unphysical and computationally expensive. To prevent this, a stochastic affectation of very low stellar mass has been implemented.
When $df_{coll}$, the variation in $f_{coll}$ in one particle between one time step and the next, is smaller than $M_{min}/M_{region}$, $df_{coll}$ is affected to the particle with a probability $\frac{M_{region}df_{coll}}{M_{min}}$. When it is higher, the probability is one. In practice, this prevents star formation at high $z$ while ensuring that the average $f_{coll}$ in the simulation converges to the theoretical value predicted by the CMF at $z \lesssim 15 \sim 20 $.




    
When the subgrid model for star formation is active, the stellar mass that is tracked throughout the simulation is an  aggregate quantity that coarsely describe the population of unresolved galaxies. While it allows for comparison with observed star formation rates at high $z$, additional modelling is required to compare the simulated results to finer observables, such as the UV luminosity functions measured at high $z$ by several instruments like  the Hubble Space Telescope of the James Webb Space Telescope (see Chapter \ref{ch1}). Specifically, one must assume a way to ascribe a fraction of the total stellar mass or total luminosity (see next section for details) to each halos in each mass bass bin of the CMF of each particle. As observed in high resolution simulations (see e.g \cite{Ocvirk2020}), we can assume in a first approximation that the spectral energy density at $1600 \AA $ is related to the host halo mass $M_{halo}$ through a power law  :

\begin{equation}
    L_{1600}(M_{halo}) = \gamma M_{halo}^\alpha
\end{equation}

\noindent where $\alpha$ is a parameter of order unity and $\gamma$ an unknown coefficient. As was found in the  CODA II simulation \cite{Ocvirk2020} over a wide range of halo masses, we adopt $\gamma = 5/3$. $L_{1600}$ is proportional to the total luminosity $L$ through $ \int_{M_{min}}^{M_{region}} L_{1600}(M) dM= \beta L$ with a coefficient $\beta$ obtained by assuming a black body spectrum and a temperature of $28000 K$ {(consistently with the source model of \textsc{Licorice})},  and  $\gamma$ is found for each particle by using the normalization condition (implied by the fact that the total $L$ is computed in \textsc{Licorice}, and this model is a way to  allocate this luminosity to halos of different masses)




\begin{equation}
    L = \frac{V_{region}}{\beta} \int_{M_{min}}^{M_{region}}  n_c(M) \gamma M^\alpha\rm{dM}
\end{equation}

 Since the CMF of each particle can be recomputed from saved snapshots, this modelling can be applied in a post-processing step with varying $\alpha$. To convert to AB1600 magnitudes $M_{UV}$, popular amongst observers, we use \citep{Oke1983b}

\begin{equation}
log_{10}(\frac{L_{1600}}{ \rm{erg s^{-1}Hz^{-1}}}) = 0.4 \times (51,64 - M_{\text{UV}})
\end{equation}


%\adr{simus 11443}
\begin{figure} [h]
    \centering
    \includegraphics[scale = 0.47]{ch2/fig/lum_func_sim11443.pdf}
    \caption{UV luminosity function of a typical simulation from the \textsc{\textsc{Loreli}} II database at $z\sim10$ (black), $z\sim8$ (red), $z\sim6$ (green), compared with observations from \cite{Oesch2018, Ishigaki2018, Atek2018}. The UV luminosity functions in \textsc{Licorice} describe unresolved structure. They are derived from the CMFs and modelling from first principle described in the text. They show a decent agreement with the observations, which is evidence for the soundness of the star formation module of \textsc{Licorice}. Credits : Matthieu Penet.  }
    \label{fig:UV lUM}
\end{figure}

As seen on Figure \ref{fig:UV lUM}, we find, at different $z$, a good agreement between observed data from \cite{Oesch2018, Ishigaki2018, Atek2018} and the UV luminosity function computed in a \textsc{Licorice} simulation calibrated so that its total SFRD is within $1\sigma$ of observations from \cite{Bouwens2016, Oesch2018, McLeod2016}. The previous discussions confirmed that the implemented CMF subgrid model and assumptions mentioned above correctly describe galaxy populations and evolution at $z \lesssim 10$.

\subsection{Radiative transfer : Monte Carlo 3D ray-tracing on a grid}\label{sec:RT}

\subsubsection{Propagating the photon packets}

The propagation of the ionizing radiation and their interaction with matter is a crucial component of the EoR. To simulate it, monochromatic photon packets are emitted from source particles (i.e. gas particles with $f_* > 0$) in random directions. The minimum and maximum numbers of photons packets emitted by each source are numerical parameters chosen to fit memory requirements and keep Monte Carlo noise to a level where its effect on 21-cm observables is small compared to e.g. the effect of the instrumental thermal noise. As the EoR requires solving radiative transfer in both the UV and X-ray bands, half of the photons sent are UV photons and half are X-rays. 

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.42]{ch2/fig/frac_ion_vs_z2048like_ST.pdf}
    \caption{Ionized fraction history of the HIRRAH-21 and LORRAH-21 simulations. The calibration of the escape fraction in LORRAH-21 allows for a good agreement with HIRRAH-21. This is the only calibration step needed for the low-resolution setup to recover the global quantities of the high-resolution one, and accounts for the lack of recombination caused by the low resolution, especially around the sources.  }
    \label{fig:frac_ion}
\end{figure}


Photon packets propagate through the simulation box at the speed of light. To process their interaction with the gas they encounter, the particles are first dispatched on an adaptive grid identical to the tree grid described in the previous section, the only difference being that the smallest RT cells contain either 0 or {fewer than} 8 particles instead of 0 or 1. $\rho_{HI,cell}$, the density of neutral hydrogen atoms of a cell is related to $\rho_{HI,part}^{(i)}$, the one of the particles it contains, through 

\begin{equation}
  \rho_{HI,cell}  =  \frac{ \sum_i \rho_{HI,part}^{(i)} V_{part}^{(i)}}{\sum_i V_{part}^{(i)}}
\end{equation}

\noindent where the sum is taken over the particles in the cell and $V_{part} = \frac{4}{3}\pi h^3 / N_{vois}$ is the volume of the particle, as calculated with SPH. When a photon packet containing $N_\gamma$ photons travels {along a path that intersects with an RT cell over a length $L_{path}$}, it deposits a number $N_{abs}$ of its photons in the cell according to 

\begin{equation}\label{eq:abs_phot}
    N_{abs} = N_\gamma(1- e^{-\tau})
\end{equation}

\noindent where $\tau = \rho_{HI, cell}L_{path} \sigma_{HI}$ is the optical depth through the cell, with $\sigma_{HI}$ the cross-section corresponding to the interaction. UV (resp. X-ray) packets with less than $1\%$ (resp. $3\%$)  of their initial energy content are killed to save computation time.  

%Each photon packet is propagated until it is killed, using a time step $\Delta t_{RT}$ smaller than the dynamical time step $\Delta t_{dyn}$, before propagating the next packet.
The properties of a cell are updated either before each dynamical time step or whenever $F_{\gamma}$, the average ionizing photon flux received since its last update, is large enough to typically ionize $\sim 10\%$ of the neutral hydrogen content of the cell, or whenever the cells undergoes net recombinations.


\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.4]{ch2/fig/avT_all_vs_z2048like_ST.pdf}
    \caption{ \cite{Meriot2024}. History of the average temperature of all particles in both LORRAH-21 and HIRRAH-21, as well as the temperature of weakly ($<2\%$) ionized particles. In the case of LORRAH-21, the temperature of the neutral phase of the particles is also shown. There again, a good agreement between LORRAH and HIRRAH is observed, both on average an in the neutral gas.}
    \label{fig:temp_vs_z}
\end{figure}

\subsubsection{Updating the cells}
 
The properties of the cell we wish to update are its ionized fraction $x_{HII}$, its average temperature $T$ and the temperature of its neutral gas  $T_{HI}$. To do so, the following coupled equations are integrated :

\begin{equation}\label{eq:xhii}
        \frac{dx_{HII}}{dt} = F_{\gamma} + \kappa_{coll} n_e (1-x_{HII})  - \kappa_{rec} x_{HII} n_e
\end{equation}

\begin{equation}\label{eq:tp}
        \frac{dT}{dt} = \frac{2}{3 k_B n}\left[ - \frac{3}{2}k_B T\frac{dn}{dt} + \Lambda + K \right]
\end{equation}


\begin{equation}\label{eq:tphi}
        \frac{dT_{HI}}{dt} = \frac{2}{3 k_B n_{HI}}\left[ - \frac{3}{2}k_B T_{HI}\frac{dn_{HI}}{dt} + \Lambda_{HI} + K_{HI} \right]
\end{equation}

\noindent where $n_e$ is the number density of electrons in the cell, $n_{HI}$ the number density of neutral hydrogen, $n$ the total number density, $\kappa_{coll}$ and $\kappa_{rec}$ the collisional ionization and recombination coefficients. $\Lambda$ represents the sum of heating and cooling terms due to X-ray heating and collisional cooling, recombination cooling, Bremsstrahlung cooling, and Compton heating caused by CMB photons \citep{Baek2009, Baek2010, BAEKth}. $\Lambda_{HI}$ represents only the effects that apply to the neutral gas; in practice, only X-ray heating is considered. $K$ is the change in internal energy of the gas particles in the cell as they expand/contract adiabatically (as well as the effect of the SPH artificial viscosity) detailed in \eqref{eq:dudt}, while $K_{HI}$ represents the same quantity for the neutral IGM. 

\subsubsection{The neutral phase of the particles}


Equation \eqref{eq:tphi} and the numerical tracking of the physical quantities within imply another form of subgrid modelling. In high resolution simulations, ionization fronts of ionized bubbles are sharp : most particles are either entirely neutral or entirely ionized. Since only the neutral particles contribute to the 21-cm signal, tracking only the average temperature of each particle is sufficient to properly compute the 21-cm brightness temperature using equation \eqref{eq:dtb}. However, in low resolution regimes, the ionization fronts are not as resolved, and many partially ionized particles can appear, even more so when the $M_{min}$ parameter is set at $\sim 10^8 \Msun$, allowing light halos and galaxies to appear in virtually all particles of the simulation at redshift $z \lesssim 10-15$.
Since the intensity of the 21-cm signal depends directly on the temperature of neutral hydrogen, its evaluation is critical. However, the ionized IGM  typically sits at $\sim 10000 \, {\rm{K}}$, while the neutral IGM, even when heated by X-ray, has a temperature of $\sim 1\, {\rm{K}}-100 \, {\rm{K}}$. Therefore, the average temperature of a partially ionized particle is greater than the actual temperature of the neutral IGM, often by orders of magnitude, leading to significant systematic bias of the 21-cm brightness temperature. To correct for this, a two-phase subgrid model for the particles was adopted. Assuming that under the resolution would lie two distinct regions, neutral and ionized, the temperature of the neutral phase is computed according to equation \eqref{eq:tphi}. $ \Lambda_{HI}$ represents X-ray heating, and $K_{HI}$ is computed following equation \eqref{eq:dudt}. %except that the index $i$ (representing the particle updated by SPH) represent the properties of the neutral IGM, and the quantities indexed by $j$ (representing the neighbour particles) are still the average properties of the neighbours. \adr{retirer derniere phrase ou detailler}




We show on Figure \ref{fig:temp_vs_z} a comparison between the thermal history of LORRAH-21 and HIRRAH-21. While the two simulations display very similar evolutions of the average temperature, the temperature of weakly ionized ($x_{HII} < 2\%$) particles clearly diverges. However, the temperature of the neutral phase of the particles evolves similarly to the weakly ionized particles of HIRRAH-21. This is consistent with the effect detailed in the previous paragraph, which causes the temperature of weakly ionized to be severely overestimated in LORRAH-21, up to approximately one order of magnitude on average compared to the temperature of the neutral phase.

Integration of equations \eqref{eq:xhii} to \eqref{eq:tphi}  occurs over a short adaptive time step $\Delta t_{cool}$, which depends on the shortest timescale over which ionization fraction or temperature typically evolve given local UV and X-ray flux. An explicit integration scheme is chosen for equation \eqref{eq:xhii} and $\eqref{eq:tp}$, while equation \eqref{eq:xhii} is integrated implicitly.
In practice, $\Delta t_{cool}$ can be up to 10000 shorter than the dynamical time step. See \cite{Baek2009} for details.




\subsubsection{The source model}

While the previous subsection describes the affectation of some amount of stellar mass to each particle, irrespective of the properties of the galaxies and clusters it represents, the radiative transfer module requires details about the underlying stellar population. The stellar sources are modelled using a Salpeter initial mass function (IMF) \citep{Salpeter} with star masses between $1.6 \Msun$ and $120 \Msun$. The total luminosity of a particle, and therefore the total spectral energy density (SED) associated with this mass distribution, are estimated by integrating over the IMF while taking into account different life times for different stellar mass bins. Finally, the frequencies of the UV photon packets are drawn from the resulting SED (see \cite{Baek2010, Meynet1997, Meynet2005}). However, not all photons emitted from stars permeate into the IGM. Most of them are absorbed by the dense gas in the interstellar medium and do not escape their host halo. To account for these photons {lost to processes below the resolution}, the total energy of the photon packets is multiplied by $f_{esc}$ a parameter representing the escape fraction of ionizing photons. This parameter is expected to vary between a few percents and $\sim 50\%$ and is set at $\sim 0.1 - 0.2$ in high resolution \textsc{Licorice} simulations so that Reionization ends at $z\sim6$. 

Note that, when unresolved halos are taken into account (in practice in low-resolution simulations), the $f_{esc}$ parameter is still only effective at the scale of the particle, and takes into account photons lost between the unresolved halos and the border of the region represented by the gas particle. However, as seen in CODA III \citep{Lewis2021} the mean free path of ionizing photons can be shorter than the typical SPH-size of a particle ($\sim 1 \Mpc$ in $256^3$ simulations in $(300 \Mpc)^3$ boxes), causing a discrepancy between the numerical value of $f_{esc}$ and the observed escape fractions of galaxies. In addition to that, low resolution simulations are underestimating the local recombination rate $R_{rec}$ compared to high resolution ones : in a given region of overdensity $\delta$, we have $R_{rec} \propto \langle\delta^2 \rangle $, but only $ \langle\delta \rangle^2$ is accessible in simulations.
All these effects imply that simulations with different resolutions but identical star formation histories will produce different ionization and thermal histories. One way to mitigate this would be to multiply the simulated $R_{rec}$ by a clumping factor $C_{rec} = \frac{\langle\delta^2 \rangle}{\langle\delta \rangle^2}$. While several approaches to estimate the clumping factor exist in the literature \citep{Kaurov2014, Mao2020, Chen2020, Bianco2021}, their implementation in our simulations failed to fully erase the dependence on resolution of the reionization timing and did not affect the difference between the thermal histories in low and high resolution simulations.
To make up for this, a local-ionization-dependent escape fraction model was implemented :

     
  \begin{align}
  f_{esc} = 
         \begin{cases}
               f_{esc, post} & {\rm{if}} \;  x_{ion} > x_{thresh}\\
              f_{esc, pre} & {\rm{if}} \; x_{ion} < x_{thresh}\\
    \end{cases}       
        \end{align}

\noindent where $f_{esc, post} = 0.1 $, $f_{esc, pre} = 0.01 $, and $x_{thresh} = 0.01 $ are parameters of this model, calibrated on HIRRAH-21 for LORRAH-21. As seen on equation \ref{fig:frac_ion}, this model allows for a good agreement between the ionization histories of the simulations. The dependence on local ionization fraction of the photon budget is motivated by the fact that at the considered resolution ($\sim 1 \Mpc$), the unresolved sources are likely to be surrounded by unresolved dense gas which must first be ionized before letting ionization photons escape into the IGM, and will exhibit a high recombination rate. This description is consistent with the short  mean free path of UV photons  found in the very high resolution simulation CODA III  (between $\sim 10^{-4} \Mpc$ and $\sim1 \Mpc$ depending on the progress of Reionization). Additional studies are required to further validate or improve the model.\\
 

Regarding the X-ray emissions, two main sources of X-rays are taken into account : Quasars (QSOs), that have strong emissions in the "soft" X-ray band ($E \leq 2 \, {\rm{keV}}$), and X-ray Binaries (XRBs), that emit "hard" X-rays. These two sources differently affects the IGM : as the soft X-rays have a mean free path of a few cMpc, they tend to heat the gas that surrounds the sources. Conversely, the harder X-rays can have a mean free path close to a cGpc. In practice, after they travel over a length greater than the size of the simulation box, they are added to a uniform background. This modelling adds inhomogeneity to the X-ray heating in the simulation, {and therefore to the 21-cm emission}. Following e.g. \cite{Furlanetto2006a}, we write $L_X$, the total X-ray luminosity of the particles 
\begin{equation}
    L_X = 3.4 \times 10^{40} f_X \left(\frac{SFR}{1 \Msun yr^{-1}}\right) \rm{erg.s^{-1} }
\end{equation}

\noindent where $f_X$ is the X-ray efficiency. As this equation is the result of observation of low-redshift galaxies, $f_X$ is a parameter that serves as a correction to model the unknown properties of high-redshift objects. The respective intensities of XRBs and QSOs are controlled using the hard-to-soft ratio $r_{H/S}$, defined as 

\begin{equation}
    r_{H/S}   = \frac{f_X^{XRB}}{f_X}  
\end{equation}

\noindent with $f_X = f_X^{XRB} + f_X^{QSO}$. The spectra of the QSOs are modelled using a simple power law with spectral index $\alpha = 1.6$ between $0.1 \, \rm{keV}$ and $2 \,\rm{keV}$, while our modelling of the XRBs use spectra drawn from \cite{Fragos2013}. Similarly to UV packets, X-ray packets propagate and deposit their energy in cells through photoionization and secondary ionizations : a number of absorbed photons $N_{abs}$ of frequency $\nu$ is estimated as in equation \ref{eq:abs_phot}, and they deposit an energy $N_ {abs}  h\nu (\nu - \nu_{ion}) f_{x,heat}$
where $f_{x,heat}$ is the fraction of the energy that is effectively converted into heat, taken from \cite{Shull1985} (see Chapter \ref{ch1}).   \\

\subsection{Simulation setup}

 The previous sections describe the simulation code in its entirety. Combining the dynamics, star formation, and RT modules, the simulations are run from $z_{init} \approx 100$, using MUSIC \citep{Hahn2011} initial conditions as a starting point and considering a recombination redshift of $z_{rec} = 130$ as predicted by the code RECFAST \citep{Seager12000}. {This determines the "initial" average gas temperature at $z = 100$, as $T(z=z_{init}) \approx 2.72 (1 + z_{init})^2 / (1 + z_{rec}) \, {\rm{K}} $}.



 
 The simulations are run until the end of Reionization, arbitrarily defined as a threshold in average ionization fraction taken at $99\%$ ionization. The computational requirements of the codes naturally depends on the numerical parameters (mainly resolution) and physical parameters : late star formation and high escape fractions typically implies fewer calls to the RT methods, varying the simulation cost by factor of $\sim2$ between extreme corners of a physically reasonable parameter space (such as the one used in the {\textsc{Loreli}} databases, described later). That being said, $2048^3 $  simulations such as HIRRAH-21 require $\sim 3 \times 10^6$ CPU-hours and are run over $4096$ MPI domains, while low-resolution ($256^3$) simulations equipped with the previously described subgrid models are typically $10 000$ cheaper and run over $64$ domains.
 
 Roughly 50 snapshots, containing the full particle data, are saved at linearly spaced time intervals, as are 3D particles light-cones. All the particle data saved during the simulation are dispatched on a grid (typically $256^3$), following an interpolation scheme with the same spline kernel function as in the SPH algorithm, shown in equation \eqref{eq:sphkern}.

\subsection{Postprocessing : the Lyman-$\alpha$ coupling}


 \begin{figure}
    \centering
    \includegraphics[scale = 0.4]{ch2/fig/wings_nowings.png}
    \caption{ From \cite{Semelin2023}. The power spectra of the 21-cm brightness temperature of several $256^3$ \textsc{Licorice} simulations are plotted at $z = 16.5$, computed with and without taking into account the wings of the Ly-$\alpha$ line. Using the wings causes a systematic increase in the spectra, up to a factor $\sim2$. The thermal noise of several instrumental setups are also plotted for comparison. }
    \label{fig:spinter_wings}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale = 0.4]{ch2/fig/spinter_vs_lico2.png}
    \caption{From \cite{Semelin2023}. Similar to Figure \ref{fig:spinter_wings} (at $z \sim12$) with additional spectra computed using the Ly-$\alpha$ radiative transfer module of \textsc{Licorice}, with and without the distortions caused by the local flow of the gas. The gas velocities cause a drop in the fluctuations of a factor $\sim 2$ at large scales and cannot be properly taken into account in the analytical formalism of \textsc{Spinter}.  }
    \label{fig:spinter_lico}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 0.3]{ch2/fig/dtb_4e9_tp_av_hi.pdf}
    \caption{Global 21-cm signal in  HIRRAH-21 and LORRAH-21, the latter calculated using either the phase-averaged temperature $\langle T \rangle$ of particles or the temperature of their neutral phase $T_{HI}$. This shows that properly taking into account the temperature of the neutral phase is critical to correctly model the 21-cm signal in low-resolution numerical simulations. From \cite{Meriot2024}. }
    \label{fig:dtb_lorrah}
\end{figure}



The last critical step required to reach the 21-cm signal is the computation of the Wouthuysen-field coupling. The first way to do it is to compute the full Lyman-$\alpha$ radiative transfer. To do so, the \textsc{Licorice} Monte Carlo ray-tracing algorithm can be run in a post-processing step on the saved snapshots to propagate Ly-$\alpha$ photon packets on a uniform grid \citep{Semelin2007}. Photons  are emitted between the $n=1$ (Lyman-$\alpha$) and $n=10$ lines of the Lyman series and are propagated and redshifted until they reach the core of the line. They then undergo a massive number of scatterings, on average $10^6$, as the gas is extremely opaque with a mean free path of the photons shorter than a pc. These scatterings are too computationally expensive to be explicitly simulated, so the spatial diffusion of the coupling due to the scattering is neglected, and $P_{\alpha}$, the number of scattering per atom per second is computed for each grid cell depending on the temperature, density, and velocity of the gas, allowing a direct computation of $x_\alpha$ (see Chapter \ref{ch1}). Monte Carlo ray tracing with \textsc{Licorice} remains a costly approach which can represent a significant fraction of the total computation time, which led to the development of semi-numerical codes such as \textsc{Spinter}, to effectively compute $x_\alpha$ at a fraction of the cost.




I briefly summarize the code here, and redirect the reader to \cite{Semelin2023} for more details. \textsc{Spinter} computes the $x_\alpha$ coupling at redshift $z$ by convolving a spherically symmetrical propagation kernel with the emissivity field evaluated at previous redshifts. If $\epsilon$ is the number of photons emitted isotropically per unit volume, time, and frequency and $n$ the number density of photons per unit frequency, they are related through the linear operator $D$ :

\begin{equation}
    D\epsilon = n
\end{equation}

It follows that $n$ can be computed using the green function $G$ of the operator $D$ :

\begin{equation}\label{eq:n_spin}
    n(\textbf{r},z,\nu) = \int \epsilon(\textbf{r},z,\nu)G(\textbf{r},z,\nu){\rm{d^3}} r {\rm{d}}\nu {\rm{d}}z
\end{equation}

In the free-streaming case in an expanding Universe, photons emitted at $\textbf{r}_0 = 0$, $\nu_0$, $z_0$ will, at redshift $z_1$, end up at a distance $r_1 = \int^{z_1}_{z_0} \frac{c}{H(z)}{\rm{d}}z$ from the emission point with frequency $\nu_1 = \frac{1 + z_1}{1 + z_0}\nu_0 $. Assuming no absorption or scattering, the number of photons is conserved, and the green function can then be written :

\begin{equation}\label{eq:green1}
    G(\textbf{r}, z_1, \nu) = \frac{1}{H(z_0)(1+z_0)4\pi r_1^2} \delta( ||\textbf{r}||-r_1) \delta( \nu - \nu_1) 
\end{equation}

Therefore, given an emission field, $n$ can be computed using equation \eqref{eq:n_spin}.  Equation \eqref{eq:green1} holds if we assume the Ly-$\alpha$ line to be a Dirac. To take into account the scatterings in the wings of the line, it must be modified. Assuming a homogeneous density field and neglecting thermal and bulk velocities, $G$ can be written as 

\begin{equation}\label{eq:green2}
    G(\textbf{r}, z_1, \nu) = F( r_1, z_1,z_0) \delta( \nu - \nu_1) 
\end{equation}

\noindent where F is an unknown function. Photon number conservation implies the normalisation condition 

\begin{equation}
     \int F( r, z_1,z_0)4\pi r^2 {\rm{dr}} = \frac{1}{H(z_0)(1+z_0)}
\end{equation}

For the Ly-$\alpha$ alpha line, \textsc{Spinter} estimates $F$ by emitting many photons around a single source in a homogeneous medium and simulating their scatterings. Assuming a spherically symmetric $F$, this simulation is fast since it is effectively $1$D. For the higher lines, the free-streaming case is used. The effect of the wing of the line on the 21-cm power spectrum at $z = 16.5$, can be seen on Figure \ref{fig:spinter_wings}, as both formalism have been run on \textsc{Licorice} data generated with different star formation parameters. On standard models of reionization, including the wings typically increases the power at all scales by a factor of $2$, enough for some models to rise above the thermal noise limits of interferometers. On average, using \textsc{Spinter} to compute a single $256^3$ $x_\alpha$ cube from \textsc{Licorice} luminosity cubes typically requires $\sim 0.5$ CPU-hour, a negligible cost compared to the simulation itself.

One difference between the \textsc{Spinter} semi-numerical computation and the \textsc{Licorice} Ly-$\alpha$ radiative transfer stems from the inclusion of the bulk velocities of the gas in the latter. The number of scatterings estimated by \textsc{Licorice} in a cell is, {in the core}, equal to the Gunn-Peterson optical depth $\tau_{GP} = \frac{3\Lambda \lambda_\alpha n_{HI}}{8 \pi H(z)}$, where $\lambda_\alpha$ is the Ly-$\alpha$ wavelength and $\Lambda$ the width of the line. The local bulk flow velocities $\textbf{v}$ are included by considering they act as a local perturbation of the Hubble flow, and a modified value of the optical depth is instead used :
\begin{equation}
  \tau_{GP, vel} =   \tau_{GP} \frac{H(z)}{H(z) + \frac{1}{3} div(\textbf{v})}
\end{equation}

The impact of the bulk velocities on the power spectrum and a comparison between \textsc{Spinter} and \textsc{Licorice} are shown on Figure \ref{fig:spinter_lico}. Typically, including the bulk flow dampens the fluctuations by a factor of $\sim 2$. For now, including the bulk flow into \textsc{Spinter} is not straight-forward, as the code heavily relies on homogeneity and static assumptions. 

For more details about the Ly-$\alpha$ processing and insights into the effect of bulk flows, the reader is redirected to \cite{Semelin2023}.


\subsection{The 21-cm observables}

Once cubes of $x_\alpha$ have been computed, they can be used to compute the spin temperature $T_s$  (see Chapter \ref{ch1}). Since $T_s$ depends on $x_\alpha$ which itself depends on the population in each of the 2 S levels of the H atom and therefore on $T_s$, the spin temperature is computed iteratively following the procedure described in \cite{Hirata2006}. 



\begin{figure}
    \centering
    \includegraphics[scale = 0.4]{ch2/fig/xionmap_256_xion_0_4.pdf}
    \caption{Slices of ionized fraction cubes of LORRAH-21 (\textit{left}) and HIRRAH-21 (\textit{right}) at $z\sim8$ and similar global ionized fraction. This comparison is there to qualitatively assess the performance and limitations of the subgrid model : while the large-scale structures are recovered in the low-resolution setup, many small-scales features are missing, potentially due to a lack of stochasticity in the star formation algorithm. Additionally, the ionization fronts are noticeably sharper in HIRRAH-21.}
    \label{fig:xionmap_lorrah}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 0.4]{ch2/fig/dtb_256_80.pdf}
    \caption{Similar to Figure \ref{fig:xionmap_lorrah}, but for the 21-cm brightness temperature at $z\sim11$, near the absorption peak of the simulations. The bubbles and heated surrounding regions are larger in LORRAH. The reasons are likely to be the same as the ones discussed on the previous plot.  }
    \label{fig:dtbmap_lorrah}
\end{figure}


Figure \ref{fig:dtb_lorrah} shows the global 21-cm signal in HIRRAH-21 and LORRAH-21. In all simulations, the $x_{\alpha}$ coupling was computed using \textsc{Spinter}. In the case of LORRAH, the brightness temperature has been calculated using both the average temperature $\langle T \rangle$
 (dashed) of each particle and using only the temperature of their neutral phase $T_{HI}$
 (solid), as tracked by equations \eqref{eq:tp} and \eqref{eq:tphi}. As expected given the discussion in \ref{sec:RT}, computing $\langle \delta T_b \rangle$ using $\langle T \rangle$ in LORRAH-21 yields a signal significantly higher than the one measured in HIRRAH-21. However, when computed with $T_{HI}$, the brightness temperature of LORRAH is fairly close to the one in HIRRAH across all redshifts, with a relative error of $\sim 10 \%$ mainly caused by an advance of $\Delta z \sim 0.15$ in the X-ray heating in LORRAH, visible on Figure \ref{fig:temp_vs_z} and mainly caused by a slight mismatch in star formation rate density between the two simulations. 




 Figure \ref{fig:xionmap_lorrah} and \ref{fig:dtbmap_lorrah} show maps of ionization fraction and 21-cm brightness temperatures of HIRRAH and LORRAH at different redshifts. In general, the large scale structures are recovered, and the low-resolution setups lacks small scale fluctuations. This is a consequence of the subgrid modelling : the star formation implementation lacks stochasticity and past some redshifts, it tends to form stellar mass in every particle in the simulation, thus smoothing the field. Small ionized bubbles are also likely to be erased by the $f_{esc}$ prescription. 
 
 {The ionization fronts are not as sharp in LORRAH-21 as in HIRRAH-21. A possible explanation stems from the successive grid to particles (during the computation of radiative transfer during the simulation run) and particles to grid (during the post processing computation of the ionization cubes) interpolations. In particular, the RT cells are larger in the low-resolution setup, which could blur the ionization field. This suggests that this aspect of the code could be improved in a future version.} 
 %and a better implementation of recombination should sharpen the ionization fronts around small scale bubbles.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%\newpage
\section{The \textsc{\textsc{Loreli}} databases}

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.38]{ch2/fig/contourplot_pval.pdf}
    \caption{p-value map of the \textsc{Licorice} star formation histories in the $(M_{min}, \tau_{SF})$ plane. The white contour is the $0.05$ level : what lies outside of it has a $>95\%$  probability to be incompatible with the observations shown on Figure \ref{fig:sfr_vs_z_lor2}. The white dots are the parameters sets used to sample this plane in the \textsc{\textsc{Loreli}} II database.}
    \label{fig:prior_sf}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[scale = 0.45]{ch2/fig/SFR_vs_z750signals.pdf}
    \caption{ {Star formation  density histories of the \textsc{\textsc{Loreli}} I simulations. We show the observational points from \cite{Bouwens2016, Oesch2018, McLeod2016}, used to define the explored parameter space. The blue dashed line shows the star formation in HIRRAH, discussed in the previous sections. } }
    \label{fig:sfr_vs_z_lor1}
\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[scale = 0.45]{ch2/fig/SFR_vs_z10000signals.pdf}
    \caption{Star formation  density histories of the \textsc{\textsc{Loreli}} II simulations. The points from \cite{Harikane2023, Chemerynska2023, Bouwens2023}, which use JWST data,  are shown but were not used to design the database as they were not available at the time. However, the \textsc{\textsc{Loreli}} II simulations are still largely consistent with JWST estimates.}
    \label{fig:sfr_vs_z_lor2}
\end{figure}



We now present the \textsc{\textsc{Loreli}}  databases. \textsc{\textsc{Loreli}} I contains 760  simulations (with a $256^3$ resolution) with different initial conditions. It heavily relies on the subgrid models described in the previous section. The star formation model uses the Extended Press-Schechter conditional mass function formalism, and only $\tau_{SF}, M_{min}$, and $f_X$ were varied. To avoid repetition, we will focus on the second version of the database, \textsc{\textsc{Loreli}} II. For a complete review of \textsc{\textsc{Loreli}} I, we redirect the reader to \cite{Meriot2024} (in appendix).

\textsc{\textsc{Loreli}} II consists in 9828 \textsc{Licorice} simulations (of $256^3$ particles in a $300 \Mpc^3$ box), generated using the Sheth-Tormen conditional mass function. Cosmology has been chosen to be consistent with Planck 2018 \citep{White2018}, and cosmological and numerical parameters are summarized in Table \ref{tab:numparam}. The database required $\sim 5 \times 10^6 $ CPU-hours and $\sim 50$ snapshots were saved for each simulation, resulting in a total volume of $1.5$ PB, including post-processed products. 
\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.45]{ch2/fig/frac_ion_vs_z10000signals.pdf}   
    \caption{Ionization histories of the \textsc{\textsc{Loreli}} II simulations as well as constraints from  \cite{Bouwens2015,Davies2018, Wang2020, Greig2024}. In these simulations, Reionization ends between $z\sim8$ and $z\sim5$.}
    \label{fig:xion_vs_z_lor2}
\end{figure}



\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
          \hline
          $H_0$ & $\Omega_0$ & $\Omega_b$ & $\Omega_\Lambda$ & $\sigma_8$  \\  
          \hline
          67.4 km/s/Mpc & 0.315 & 0.0492 & 0.685  & 0.811  \\
          \hline
  \end{tabular}
 \hspace{15.5cm}
  
    \begin{tabular}{|c|c|c|}
          \hline

          $L_{box} (\Mpc)$ & dt (Myr) & $N_{part}$ \\
          \hline

          294 & 7 & $256^3$\\ 
          \hline

    \end{tabular}
    \caption{Numerical and cosmological parameters of \textsc{\textsc{\textsc{Loreli}}} simulations. }
    \label{tab:numparam} 
\end{table}

The star formation parameters are strongly degenerate. To define the region in parameter space we explore in \textsc{\textsc{Loreli}} II, we use the star formation rate density observations at $z\lesssim 10$ from \cite{Bouwens2016, Oesch2018, McLeod2016}. $\tau_{SF}$ and $M_{min}$ were varied on a square grid with $\tau \in [1, 17] \rm{Gyr}$ and $M_{min} \in [10^8, 4\times 10^9] \Msun $. A $\chi^2$ test was then performed to exclude star formation histories that had a probability to be incompatible with all observation sets higher than $0.95$. The result is the white-contoured region on Figure \ref{fig:prior_sf}, which we sample with the 42 $(\tau_{SF}, M_{min})$ pairs indicated by the white dots. {A similarly constrained contour was sampled for \textsc{\textsc{Loreli}} I; it is slightly different from the one on Figure \ref{fig:prior_sf} as the star formation model differ in the two versions of the database. }  




The resulting star formation densities are shown on Figure \ref{fig:sfr_vs_z_lor1} {for \textsc{\textsc{Loreli}} I and \ref{fig:sfr_vs_z_lor2} for \textsc{\textsc{Loreli}} II }, as well as the observations used to constrain the databases. The observations in red at $z \gtrsim 10$ are taken from \cite{Harikane2023, Chemerynska2023, Bouwens2023}. They use data from the James Webb Space Telescope and were not available when the database was designed. However, the SFRD in \textsc{\textsc{Loreli}} II are still fairly consistent with these measurements. The observation at $z \sim 16$ does suggest a flatter SFRD history than what our model allows, which, if confirmed, would require either a lower $M_{min}$ (and thus taking into account molecular cooling processes) or, for instance, redshift dependent values for $\tau_{SF}$ to represent a transition from pop III to pop II stars. {Note that these SFRD are fairly uncertain and inferred from a limited number of very bright objects. }

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.37]{ch2/fig/opticaldepth_vs_z_10000signals.pdf}   
    \caption{Optical depth of the \textsc{\textsc{Loreli}} II simulations. Measurements by Planck 2015 and 2018 are also reported \citep{White2018, Ade2016}. The \textsc{\textsc{Loreli}} simulations are within $3 \sigma$ of these constraints, although they were not used to calibrate the database per se.}
    \label{fig:tau_vs_z_lor2}
\end{figure}

The escape fraction $f_{esc,post}$ takes three values in \textsc{\textsc{Loreli}} II : 0.05, 0.275, 0.5.
Previous studies have poorly constrained $f_{esc}$ and values between $\sim 0.01$ and $\sim 0.5$ have been reported (e.g. \cite{Wood1999, Iwata2009, Paardekooper2011,wise2009} ). Additionally, our parameter is defined at a scale of a particle (i.e. $\sim 1 \Mpc)$ and depends on local ionization, as previously detailed, which may differ from what observers directly access. The range of values we use is loosely defined in order to get plausible reionization timings.
The resulting ionization histories are shown on Figure \ref{fig:xion_vs_z_lor2}. As expected, Reionization ends in all simulations between $z \sim 5 $ and $z \sim 8$. Our reionization histories are within $\sim 2 \sigma$ of available constraints and upper limits from \cite{Bouwens2015,Davies2018, Wang2020, Greig2024}.
We calculate the Thomson optical depth $\tau_T$ following 



\begin{equation}
    \tau_T = c \sigma_T \int_0^z \frac{n_e(z) \rm{dz}}{(1+z)H(z)}
\end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.38]{ch2/fig/dtb_10000signals.pdf}
    \caption{Average global $\delta T_b$ of the 10000 \textsc{\textsc{Loreli}} II simulations, colour coded according to the X-ray intensity parameter $f_X$. The most intense signals reach $\sim -220 \, {\rm{mK}}$ at $z \sim 8$, far from the EDGES measurement at $-500 \, {\rm{mK}} $ at $z \sim 16$.}
    \label{fig:dtb_vs_z_lor2}
\end{figure}

Assuming a second Helium ionization at $z=3$. The results are shown on Figure \ref{fig:tau_vs_z_lor2}, as well as values measured by the Planck collaboration \citep{White2018}. It must be noted that our simulated ionization histories shapes may differ from the ones assumed in the Planck analysis. For this reason, we report the highest and lowest $\tau_T$ values from 2018 Planck results.  Our results are within $\sim3 \sigma$ of these measurements, even our late-reionization scenarios. \\







As almost no constraint exist on X-ray emissions of high-z galaxies, we vary the corresponding parameters over wide ranges :  $f_x \in [0.1,10]$ (13 logarithmically spaced values), and  $r_{H/S}  \in [0,1]$, (6 linearly spaced values). However, after the design of this simulation project, a few AGNs have been detected by JWST that suggest a $f_X$ higher than $10$ and closer to $100$ at $z\sim4$ \citep{Kocevski2023}. As the JWST can only detect the brightest objects (typically with $f_X > 10$), these measurements might not accurately represent the average galaxies at high redshift. On the other hand, the SKA pathfinders will first constrain the most intense 21-cm signals, which are typically caused by a low $f_X$, and $f_X \sim 0.1$ allows us to investigate scenarios with almost no heating. 




To save computation time, simulations were post-processed using \textsc{Spinter} and including the effect of the wings of the Lyman-$\alpha$ line. {Roughly 500 000 cubes of 21-cm brightness temperatures $\delta T_b$ were then computed at $256^3$ resolution}, as well as the corresponding 21-cm power spectra. Figure \ref{fig:dtb_vs_z_lor2} shows the global $\delta T_b$ of all simulations, colour coded to display their clear dependence on $f_X$. As these models do not include any exotic physics, they are far from matching the EDGES signal, characterized by a sharp and deep absorption feature  ($\sim -500 \pm 200$ mK) at $z\sim16$. However, some exotic models (such as an excess radio background \citep{Fialkov2019}) can be implemented in post-processing steps if needed. For now, since EDGES signal has not been reproduced by subsequent global signal experiment SARAS3, including EDGES-like signals in the project was not deemed a priority. 


\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.6]{ch2/fig/powerspectra_loreli2_vs_z_k01.pdf}
    \caption{Power spectra of the \textsc{\textsc{Loreli}} II simulations at $k\sim0.1 \, {\rm{h.Mpc^{-1}}}$ as a function of $z$, compared to theoretical sensitivities of NenuFAR and LOFAR. Recent upper limits from \cite{Patil2017, Mertens2020, Trott2020,TheHERACollaboration2022} are also shown. HERA results are likely to slightly constrain the database parameter space. }
    \label{fig:pk_vs_z_lor2}
\end{figure}



\begin{figure}[h!]

    \centering

    \includegraphics[scale = 0.4]{ch2/fig/powerspectra10000_z14-1.png}
    %\caption{$k\sim0.1$}
    
% \end{figure}
% \begin{figure}

\begin{minipage}[left]{.45\textwidth}        

    \includegraphics[scale = 0.4]{ch2/fig/powerspectra10000_z10.pdf}
    %\label{fig:pk_vs_k_lor2_2}
    \hspace{.1\textwidth}
     
\end{minipage}
\begin{minipage}[right]{.45\textwidth}
        \hspace{.08\textwidth}
        \includegraphics[scale = 0.4]{ch2/fig/powerspectra10000_z8.pdf}
    %\label{fig:pk_vs_k_lor2_3}

        \end{minipage}
    \caption{\textsc{\textsc{Loreli}} II power spectra as a function of $k$ at different redshifts. The expected SKA thermal noise for 1000h of observations is also plotted, proving that the instrument can very easily detect our models. The figures also display a transition from a coupling-driven signal to a heating-driven one.}
\label{fig:pk_vs_k_lor2_1}
\end{figure}

Figure \ref{fig:pk_vs_z_lor2} shows the evolution of the \textsc{\textsc{Loreli}} II power spectra at $k\sim0.1 \, {\rm{h.Mpc^{-1}}}$, as well as current upper limits from various interferometers. The expected sensitivities of LOFAR and NenuFAR (for 1000h of observations) are also plotted. While LOFAR should be able to detect most of the \textsc{\textsc{Loreli}} II signals, NenuFAR can only hope to constrain exotic models.
Most instrumental upper limits on the signal are roughly an order of magnitude too high to be able to exclude our simulations, except for the 2022 HERA data, which may constrain the most intense signals, characterized by a low $f_X$. See Chapter \ref{chp3_chap} section \ref{sec:inf_hera}  for further discussion.
Figure \ref{fig:pk_vs_k_lor2_1} shows the spectra at different redshifts, giving a sense of the orders of magnitude of the data, illustrating that they should be easily distinguished by the SKA, and how the intensity of the fluctuations are initially mostly caused the star formation parameters, before switching to a regime where $f_X$ dominates. \\

We have introduced the \textsc{Licorice} simulation code and the modifications that made it possible to create the \textsc{\textsc{Loreli}} I and II databases, first of their kind in the 21-cm community. The modelling of the EoR is arduous, and so can be the comparison of the theoretical predictions with observational data. In the next chapter, we explain how the \textsc{\textsc{Loreli}} databases can be used to interpret current and future measurements of the 21-cm power spectrum and devise constraints on the parameters in our astrophysical models.


\newpage

% \begin{figure}
%     \centering
%     \includegraphics[scale = 0.5]{ch2/fig/powerspectra10000_z8-1.png}
%     \caption{$k\sim0.1$}
%     \label{fig:pk_vs_k_lor2_3}
% \end{figure}


% \subsection{Paragraph a grid;e avec une figure}

% \lipsum[50]
% \begin{figure}[H]\centering
% \includegraphics[width=.5\linewidth]{ch2/fig/Saturation_voxel_size.png}
% \caption{Une description avec la légende associée et sa référence.}
% \label{fig2_example}
% \end{figure}

% \subsection{Résultats avec un tableau}
% \lipsum[51]

% \begin{table}[H]\centering
% \begin{tabular}{lcc}
%                                  & \textit{In silico} & \textit{In vitro} \\ \hline
% Number of half cycles            & 2        & 4                    \\ \hline
% Duty cycle                       & \SI{33}{\%}     & \SI{45}{\%}                 \\ \hline
% \end{tabular}
% \caption{Un exemple de tableau}\label{tab2_num1}
% \end{table}

